Identification of asteroids using the Virtual Observatory: the WFCAM Transit Survey

The nature and physical properties of asteroids, in particular those orbiting in the near-Earth space, are of scientific interest and practical importance. Exoplanet surveys can be excellent resources to detect asteroids, both already known and new objects. This is due their similar observing requirements: large fields of view, long sequences, and short cadence. If the targeted fields are not located far from the ecliptic, many asteroids will cross occasionally the field of view. We present two complementary methodologies to identify asteroids serendipitously observed in large-area astronomical surveys. One methodology focuses on detecting already known asteroids using the Virtual Observatory tool SkyBoT, which predicts their positions and motions in the sky at a specific epoch. The other methodology applies the ssos pipeline, which is able to identify known and new asteroids based on their apparent motion. The application of these methods to the 6.4 deg 2 of the sky covered by the Wide-Field CAMera Transit Survey in the J-band is described. We identified 15 661 positions of 1 821 different asteroids. Of them, 182 are potential new discoveries. A publicly accessible online, Virtual Observatory compliant catalogue was created. We obtained the shapes and periods for five of our asteroids from their light-curves built with additional photometry taken from external archives. We demonstrated that our methodologies are robust and reliable approaches to find, at zero cost of observing time, asteroids observed by chance in astronomical surveys. Our future goal is to apply them to other surveys with adequate temporal coverage.

==> spin_results_RoPACS.tex <==
 23967 & 1998 XQ12                 &   190 & $-18$ &   357 & $-45$ &  5.47479 &             &       \\
 32748 & 1981 EY7                  &   107 &    29 &   276 &    49 &  9.53678 &             &       \\
 44217 & Whittle                   &    63 &    51 &   216 &    34 &  9.78271 &         9.7$\pm$0.1 &     2 \\
102913 & 1999 XT21                 &   201 & $-23$ &       &       &  15.9591 &             &       \\
245376 & 2005 GC79                 &     6 &    33 &       &       &  7.93897 &             &       \\

